The (In)Efficiency of Interaction

Evaluating higher-order functional programs through abstract machines inspired by the geometry of the interaction is known to induce $\textit{space}$ efficiencies, the price being $\textit{time}$ performances often poorer than those obtainable with traditional, environment-based, abstract machines. Although families of lambda-terms for which the former is exponentially less efficient than the latter do exist, it is currently unknown how \emph{general} this phenomenon is, and how far the inefficiencies can go, in the worst case. We answer these questions formulating four different well-known abstract machines inside a common definitional framework, this way being able to give sharp results about the relative time efficiencies. We also prove that non-idempotent intersection type theories are able to precisely reflect the time performances of the interactive abstract machine, this way showing that its time-inefficiency ultimately descends from the presence of higher-order types.

==> 99-14_-_Space.tex <==
% !TeX spellcheck = en_US
% !TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proofs of \refsect{space} (The Space (In)Efficiency of Interaction)}

\begin{proposition}
	Let $\tmthree_k^h$ be a term defined as 
	$\tmthree_k^h=(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo 
	z)\tm_1...\tm_k(\la w{w\tmtwo_1\,...\tmtwo_h})$. The the $\IAM$ space 
	consumption for the evaluation of $\tmthree_k^h$ is 2 
	logged positions plus $h+k$ occurrences of $\resm$, while the $\JAM$ needs 
	2 logged positions plus $\max\{h,k+1\}$ occurrences of	$\resm$.
\end{proposition}
\begin{proof}
	If we evaluate $\tmthree_k^h$ with the 
	$\IAM$, we have the following sequence of reductions:
	\[
	\begin{array}{rcl}
	\dstate{\tmthree_k^h}{\ctxhole}{\stempty}{\stempty}&\toiam^{k+1}& 
	\dstate{\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo z} 
	{\ctxhole\tm_1...\tm_k(\la 
		w{w\tmtwo_1\,...\tmtwo_h})}{\resm^{k+1}}{\stempty}\\
	&\toiam^{k+2}&\dstate{\vartwo}{(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\ctxhole
		z)\tm_1...\tm_k(\la w{w\tmtwo_1\,...\tmtwo_h})}{\resm}{\stempty}\\
	&\toiam^{k+1}&\ustate{\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo 
		z} {\ctxhole\tm_1...\tm_k(\la 
		w{w\tmtwo_1\,...\tmtwo_h})}{\resm^{k}\cons(\vartwo,\la\vartwo\ctxhole,\stempty)\cons\resm}{\stempty}\\
	&\toiam^{k+1}&\dstate{\la 
		w{w\tmtwo_1\,...\tmtwo_h}}{(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo
		z)\tm_1...\tm_k\ctxhole}{\resm}{(\vartwo,\la\vartwo\ctxhole,\stempty)}\\
	&\toiam^{h+1}&\dstate{w}{(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo
		z)\tm_1...\tm_k(\la 
		w{\ctxhole\tmtwo_1\,...\tmtwo_h})}{\resm^h}{(\vartwo,\la\vartwo\ctxhole,\stempty)}\\
	&\toiam&\ustate{\la 
		w{w\tmtwo_1\,...\tmtwo_h}}{(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo
		z)\tm_1...\tm_k\ctxhole}{(w,\la
		w\ctxhole\tmtwo_1\,...\tmtwo_h)\cons\resm^h}{(\vartwo,\la\vartwo\ctxhole,\stempty)}\\
	\textsf{BT}&\toiam^{k+1}&\dstate{\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo
		z}{\ctxhole\tm_1...\tm_k(\la 
		w{w\tmtwo_1\,...\tmtwo_h})}{\resm^k\cons(\vartwo,\la\vartwo\ctxhole,\stempty)\cons(w,\la
		w\ctxhole\tmtwo_1\,...\tmtwo_h)\cons\resm^h} 
	{\stempty}\\
	\textsf{BT}&\toiam^{k+1}&\ustate{\vartwo}{(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo
		\ctxhole z)\tm_1...\tm_k(\la 
		w{w\tmtwo_1\,...\tmtwo_h})}{(w,\la 
		w\ctxhole\tmtwo_1\,...\tmtwo_h)\cons\resm^h} 
	{\stempty}\\
	&\toiam&\dstate{z}{(\lambda{\var_1}...\lambda{\var_k}.\la\vartwo\vartwo
		\ctxhole)\tm_1...\tm_k(\la 
		w{w\tmtwo_1\,...\tmtwo_h})}{\resm^h} 
	{(w,\la w\ctxhole\tmtwo_1\,...\tmtwo_h)}\\
	\end{array}
	\]
	The space consumption is thus the maximum size reached by states \ie\ 2 
	logged positions plus $h+k$ occurrences of $\resm$. Evaluating the term 
	with $\JAM$ avoids 
	the backtracking phase, highlighted with the \textsf{BT} label, which is 
	when the maximum size is reached during the $\IAM$ computation. In 
	particular, the $\JAM$ consumes 2 logged positions plus $\max\{h,k+1\}$ 
	occurrences of	$\resm$.
\end{proof}

==> latex-macros/ben-macros-nets.tex <==
%% tikz
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations.shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning}
\usepackage[nofancy]{tikz-inet}

\setboolean{withimages}{true}

\tikzset{%
%
% tikzpictures
  ocenter/.style={baseline={([yshift=-.5ex, xshift=-.5ex]current bounding box)}},  
%
% NODE STYLES
  nospace/.style={inner sep= 0pt},
  etic/.style={inner sep= 0.5pt, fill=white, anchor= center},
  letic/.style={inner sep= 0.7pt, fill=white, anchor= center,circle,draw=black},
%
% MELL nets  
  port/.style={inner sep= 0.3pt, anchor= center,circle,draw=black,fill=black, minimum size = 0.3pt},
%
% cbv nets  
  eport/.style={inner sep= 0.8pt, anchor= center,circle,draw=cyan,fill=white, minimum size = 0.8pt},
  mport/.style={inner sep= 0.8pt, anchor= center, circle,draw=white,fill=brown, minimum size = 0.8pt, solid, 
line width=0.10ex},
% cbn nets  
  eportn/.style={inner sep= 0.8pt, anchor= center,circle,draw=blue,fill=white, minimum size = 0.8pt},
  mportn/.style={inner sep= 0.8pt, anchor= center, circle,draw=red,fill=red, minimum size = 0.8pt, solid, 
line width=0.10ex},
%
%
% EDGE STYLES
  nopol/.style={->, shorten <=0.5pt, shorten >=0.5pt, draw=gray, line width=0.18ex},
  nopolrev/.style={<-, shorten <=1pt, shorten >=1pt, draw=gray, line width=0.18ex},
  nopolgen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=gray,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=0.5pt, shorten >=0.5pt, draw=gray, line width=0.18ex},
  nopolrevgen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=gray,-](0pt,3pt) -- (0pt,-3pt);}},<-, shorten <=1pt, shorten >=1pt, draw=gray, line width=0.18ex},
  outEdge/.style={<-, shorten >=0.5pt, shorten <=0.5pt, draw=blue, line width=0.18ex},
  inpEdge/.style={->, densely dotted, shorten >=0.5pt, shorten <=0.5pt, draw=red, line width=0.18ex, overlay},
  inpEdgeGen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=red,-](0pt,3pt) -- (0pt,-3pt);}},->, densely dotted, shorten >=0.5pt, shorten <=0.5pt, draw=red, line width=0.18ex, overlay},
  %
  % cbv nets
    eprinc/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=cyan, fill=cyan, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprinc/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=brown, fill=brown, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincpar/.style={postaction={decorate},decoration={markings,mark=at position .6 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=brown, fill=brown, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    pure/.style={->, shorten <=1pt, shorten >=1pt, draw=brown, line width=0.18ex},
    pureRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=brown, line width=0.18ex},
    exppure/.style={->, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},
    exppureRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},    genexppure/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=cyan,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},
    enaryedge/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=cyan,-](0pt,3pt) -- (0pt,-3pt);}}},
  % cbn nets
    eprincn/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=blue, fill=blue, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincn/.style={postaction={decorate},decoration={markings,mark=at position .6 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=red, fill=white, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincnpar/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=red, fill=white, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    puren/.style={->, shorten <=1pt, shorten >=1pt, draw=red, line width=0.18ex},
    purenRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=red, line width=0.18ex},
    exppuren/.style={->, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},
    exppurenRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},    genexppuren/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=blue,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},
    enaryedge/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=blue,-](0pt,3pt) -- (0pt,-3pt);}}},
%
% BOX LINE STYLES
  jboxline/.style={draw= gray,rounded corners, line width=0.20ex, overlay},
  exboxline/.style={draw= gray,line width=0.20ex, overlay},
  noboxline/.style={draw= white,rounded corners, line width=0ex},
%
% NETS
  net/.style={draw=gray,inner sep=2pt,thick,ellipse, anchor=center, font=\scriptsize},
  inductiveTr/.style={draw=black!50, minimum size=0.9cm},
  inductiveTrSmall/.style={draw=black!50, minimum size=0.6cm},
%
% EVERY
  every label/.style={label distance = 1pt, font=\scriptsize, inner sep= 1pt},  
  every node/.style={font=\scriptsize }%\small
}
%\node[etic,fill=white]{{\tiny 0}}

\newcommand{\altax}{8pt}
\newcommand{\altcut}{8pt}


\newcommand{\staltb}{30pt}
\newcommand{\stlarb}{25pt}
\newcommand{\hstaltb}{\staltb/2}
\newcommand{\hstlarb}{\stlarb/2}

\newcommand{\stalt}{22pt}
\newcommand{\stlar}{15pt}
\newcommand{\hstalt}{\stalt/2}
\newcommand{\hstlar}{\stlar/2}
\newcommand{\hhstalt}{\stalt/4}
\newcommand{\hhstlar}{\stlar/4}

\newcommand{\staltm}{17.8pt}
\newcommand{\stlarm}{13.6pt}
\newcommand{\hstaltm}{\staltm/2}
\newcommand{\hstlarm}{\stlarm/2}

\newcommand{\ilar}{12pt}
\newcommand{\hilar}{\ilar/2}

\newcommand{\auxdistance}{5pt}
\newcommand{\pendingdist}{10pt}
\newcommand{\anchorh}{9pt}
\newcommand{\anchorw}{9pt}

%LINKS
\input{\macrospath/graphical-macros/generic-links}
\input{\macrospath/graphical-macros/links-MELL}

%SEPARATORI
\newcommand{\invsep}[2]{%parametri: #1=larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up.center) [below right=#2 and #1](down){};
  \end{tikzpicture}
}

\newcommand{\sepColonne}[2]{%parametri: #1=larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up) [below=#2](down){};
    \draw [color=gray] (up) to (down);
    \node at (up) [left = #1] (left){};
    \node at (up) [right= #1] (right){};
  \end{tikzpicture}
}

\newcommand{\sepRows}[2]{%parametri: #1=Larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up) [right=#1](down){};
    \draw [color=gray] (up) to (down);
    \node at (up) [above = #2] (left){};
    \node at (up) [below= #2] (right){};
  \end{tikzpicture}
}

\newcommand{\lineasep}{\multicolumn{6}{c}{\sepRows{200pt}{0.5pt}}}
\newcommand{\lineaseplong}{\multicolumn{9}{c}{\sepRows{350pt}{0.5pt}}}

\newcommand{\gdots}[3]{
% 1 = left node
% 2 = right node
% 3 = eventual parameters
\node at ($(#1)!.5!(#2)$) [#3]{\tiny $\ldots$};
}

\newcommand{\gdotsname}[4]{
% 1 = left node
% 2 = right node
% 3 = eventual parameters
% 4 = name of the node
\node at ($(#1)!.5!(#2)$) [#3](#4){\tiny $\ldots$};
}

\newcommand{\bracketup}[5]{
% 1 = left node
% 2 = right node
% 3 = height
% 4 = label
% 5 = name
\node at \med{#1}{#2}[above=#3, nospace](#4){};

\draw[out=90, in=-90] (#1) to (#4);
\draw[out=90, in=-90] (#2) to (#4);
\node at (#4.center)[ above=\sepbox, nospace](#4label){#5};
}

\newcommand{\bracketdown}[5]{
% 1 = left node
% 2 = right node
% 3 = height
% 4 = label
% 5 = name
\node at \med{#1}{#2}[below=#3, nospace](#4){};

\draw[out=-90, in=90] (#1) to (#4);
\draw[out=-90, in=90] (#2) to (#4);
\node at (#4.center)[ below=\sepbox, nospace](#4label){#5};}

\newcommand{\mednop}[2]{
$(#1)!.5!(#2)$
}

==> latex-macros/graphical-macros/generic-links.tex <==
%%%%%%%%%%%%%%%%
%% AXIOM
%%%%%%%%%%%%%%%

\newcommand{\axnode}[5]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){ #5$\ax$};}

\newcommand{\axedges}[5 ]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = left edge line style
% 5 = right edge line style
\draw[#4, in=90, out=180] (#3) to (#1);
\draw[#5, in=90, out=0] (#3) to (#2);
}

\newcommand{\laxabstract}[7]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
% 6 = left edge line style
% 7 = right edge line style
\axnode{#1}{#2}{#3}{#4}{#5}
\axedges{#1}{#2}{#3}{#6}{#7}
}

%%%%%%%%%%%%%%%%
%% CUT
%%%%%%%%%%%%%%%

\newcommand{\cutnode}[5]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
\node at ($(#1.center)!.5!(#2.center)$) [below = #4, etic] (#3){ #5$\cut$};}

\newcommand{\cutedges}[5 ]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = left edge line style
% 5 = right edge line style
\draw[#4, out=-90, in=180] (#1) to (#3);
\draw[#5, out=-90, in=0] (#2) to (#3);
}

\newcommand{\lcutabstract}[7]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
% 6 = left edge line style
% 7 = right edge line style
\cutnode{#1}{#2}{#3}{#4}{#5}
\cutedges{#1}{#2}{#3}{#6}{#7}
}


%%%%%%%%%%%%%%%%
%% ZERARY
%%%%%%%%%%%%%%%

\newcommand{\lZeroary}[5]{
% 1 = one principal port	
% 2 = name of the link
% 3 = link symbol
% 4 = distance link-node
% 5 = type of edge
\node at (#1.center) [above= #4, etic] (#2){#3};
\draw[#5] (#2) to (#1);}


%%%%%%%%%%%%%%%%
%% UNARY
%%%%%%%%%%%%%%%

\newcommand{\lUnarySymbol}[5]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link, 
% 4 = link symbol
% 5 = node style
\node at ($(#2.center) ! .5 ! (#1.center)$) [#5] (#3){ #4};
}

\newcommand{\lUnary}[5]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = edge line
\lUnarySymbol{#1}{#2}{#3}{#4}{etic}

\draw[#5] (#2) to (#3);
\draw[#5] (#3) to (#1);
}

\newcommand{\lUnaryDiffEdges}[6]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = bottom edge line
% 6 = top edge line 

% symbol
\lUnarySymbol{#1}{#2}{#3}{#4}{etic}

% bottom edge
\draw[#5] (#3) to (#1);

%above edge
\draw[#6] (#2) to (#3);
}

\newcommand{\lUnaryDiffEdgesCircle}[6]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = bottom edge line
% 6 = top edge line 

% symbol
\lUnarySymbol{#1}{#2}{#3}{#4}{letic}

% bottom edge
\draw[#5] (#3) to (#1);

%above edge
\draw[#6] (#2) to (#3);
}

\newcommand{\lUnaryDiffEdgesCircleNode}[7]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = link symbol
% 5 = bottom edge line
% 6 = top edge line 
% 7 = node parameters

% symbol
\lUnarySymbol{#1}{#2}{#3}{#4}{#7}

% bottom edge
\draw[#5] (#3) to (#1);

%above edge
\draw[#6] (#2) to (#3);
}


%%%%%%%%%%%%%%%%
%% BINARY
%%%%%%%%%%%%%%%

\newcommand{\lBinSymbol}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = node style
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [#6] (#4){#5};
}

\newcommand{\lBinSymbolFixR}[6]{
% parameters
% 1 =  principal port,
% 2 = left auxiliary port,
% 3 = right auxiliary port,
% 4 = name of the link, 
% 5 = link symbol
% 6 = node style
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, #6] (#4){#5};
}

\newcommand{\lBinSymbolFixL}[6]{
% parameters
% 1 =  principal port,
% 2 = left auxiliary port,
% 3 = right auxiliary port,
% 4 = name of the link, 
% 5 = link symbol
% 6 = node style
\node at ($(#1.center) ! .5 ! (#3 -| #2)$) [below= 1pt, #6] (#4){#5};
}


\newcommand{\lBinEdgesAbove}[5]{
% 1 = left auxiliary port	
% 2 = right auxiliary port	
% 3 = name of the link
% 4 = left edge type
% 5 = right edge type
\draw[#4, in=150, out=-90] (#1) to (#3);
\draw[#5, in=30, out=-90] (#2) to (#3);
}

\newcommand{\lBinEdgesBelow}[5]{
% 1 = left auxiliary port	
% 2 = right auxiliary port	
% 3 = name of the link
% 4 = left edge type
% 5 = right edge type
\draw[#4, in=210, out=90] (#1) to (#3);
\draw[#5, in=-30, out=90] (#2) to (#3);
}


\newcommand{\lBinaryWithEdgeAboveTypes}[8]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = principal edge type
% 7 = left premise edge type
% 8 = right premise edge type
\lBinSymbol{#1}{#2}{#3}{#4}{#5}{etic}

% upper edges of the link
\lBinEdgesAbove{#2}{#3}{#4}{#7}{#8}

\draw[#6] (#4) to (#1);
}

\newcommand{\lBinaryWithEdgeBelowTypes}[9]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = principal edge type
% 7 = left premise edge type
% 8 = right premise edge type
% 9 = node style
\lBinSymbol{#1}{#2}{#3}{#4}{#5}{#9}

% upper edges of the link
\lBinEdgesBelow{#2}{#3}{#4}{#7}{#8}

\draw[#6] (#4) to (#1);
}


\newcommand{\lBinary}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = edge type
\lBinaryWithEdgeAboveTypes{#1}{#2}{#3}{#4}{#5}{#6}{#6}{#6}
}

\newcommand{\lBinaryFlipped}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = edge type
\lBinaryWithEdgeBelowTypes{#1}{#2}{#3}{#4}{#5}{#6}{#6}{#6}{etic}
}


%%%%%%%%%%%%%%%%
%% BOXES
%%%%%%%%%%%%%%%

\newcommand{\stboxlw}{6pt}
\newcommand{\stboxh}{20pt}
\newcommand{\stboxrw}{30pt}
\newcommand{\stboxrwaux}{35pt}
\newcommand{\sepbox}{2pt}
\newcommand{\belowbox}{\stboxh+2*\sepbox+1pt}

\newcommand{\boxnodes}[4]{
% 1 = link to box
% 2 = left width
% 3 = right width 
% 4 = height
\node at (#1.center)[left = #2,nospace](#1so){};
\node at (#1.center)[right = #3,nospace](#1se){};
\node at (#1se.center)[above=#4,nospace](#1ne){};
\node at (#1ne-|#1so)[nospace](#1no){};}

\newcommand{\BoxNodesWithPalOnTopAndVeticalNodeBound}[4]{
% 1 = upper node (pal of ! link) 
% 2 = bottom node 
% 3 = box left width
% 4 = box right width
\node at (#1.center)[left = #3,nospace](#1no){};
\node at (#1.center)[right = #4,nospace](#1ne){};
\node at (#1no|-#2)[nospace](#1so){};
\node at (#1ne|-#2)[nospace](#1se){};
}


\newcommand{\boxline}[2]{
% 1 = box link
% 2 = line style
\draw[#2](#1.center) -- (#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center);}

\newcommand{\BoxLineWithPalOnTop}[2]{
% 1 = box link
% 2 = line style
\draw[#2](#1so.center) -- (#1se.center) -- (#1ne.center) -- (#1.center) -- (#1no.center) -- (#1so.center); 
}

\newcommand{\abox}[5]{
% 1 = link to box
% 2 = line style
% 3 = right width 
% 4 = left width
% 5 = height
\boxnodes{#1}{#3}{#4}{#5}
\boxline{#1}{#2line}}

\newcommand{\aBoxWithPalOnTopAndVeticalNodeBound}[5]{
% 1 = upper node (pal of ! link) 
% 2 = bottom node 
% 3 = line style
% 4 = box left width
% 5 = box right width
\BoxNodesWithPalOnTopAndVeticalNodeBound{#1}{#2}{#4}{#5}
\BoxLineWithPalOnTop{#1}{#3line}
}


\newcommand{\boxauxnodes}[3]{
% 1 = link to box
% 2 = distance of the right conclusion from SE corner
% 3 = distance between the two conclusions
\node at (#1se.center)[left = #2, nospace](#1auxk){};
\node at (#1auxk.center)[left= #3, nospace](#1aux1){};
}

% \newcommand{\boxauxnodes}[2]{
% % 1 = link to box
% % 2 = box right width
% \node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
% \node at (#1auxk.center)[left= ((#2)/2), nospace](#1aux1){};
% }

\newcommand{\boxauxnodeslab}[4]{
% 1 = link to box
% 2 = left label,
% 3 = right label,
% 4 = height delta
\node at (#1auxk.center)[below = #4,etic](#1auxktarget){\tiny #3};
\node at (#1aux1.center)[below = #4,etic](#1aux1target){\tiny #2};

\draw[nopol] (#1auxk) to (#1auxktarget);
\draw[nopol] (#1aux1) to (#1aux1target);
}

\newcommand{\boxlabel}[2]{
% 1 = box link
% 2 = label
\node at ($(#1so)!.5!(#1ne)$) {#2};
}

\newcommand{\boxlineor}[3]{
% 1 = box link
% 2 = line style
% 3 = jolly point on the right
\draw[#2, overlay](#1.center) -- (#1-|#3)--(#3.center)--(#3-|#1se.center)--(#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center);}


\newcommand{\aboxor}[7]{
% 1 = link to box
% 2 = box kind
% 3 = box left width
% 4 = box right width
% 5 = box height
% 6 = label 
% 7 = jolly point
\boxnodes{#1}{#3}{#4}{#5}
\boxlineor{#1}{#2line}{#7}
\boxlabel{#1}{#6}}


%%%%%%%%%%%%%%%%
%% CONTRACTION AND WHYNOT TREES
%%%%%%%%%%%%%%%
\newcommand{\whyntreelength}{1.8*\stlar}
\newcommand{\whyntreeheigth}{1.2*\stalt}

\newcommand{\whyntreeabstract}[3]{
% 1 = principal node
% 2 = tree height
% 3 = tree base length/2
\node at (#1.center) [above left = #2 and #3, nospace](#1_left_vertex){};
\node at (#1.center) [above right = #2 and #3, nospace](#1_right_vertex){};

\draw[exboxline](#1.center) -- (#1_left_vertex.center) -- (#1_right_vertex.center) -- (#1.center);

% label
\node at (#1.center) [above=3*#2/5,nospace](#1_label){\tiny $T_{\contrp}$};

% ghost nodes for leaves
\node at (#1.center) [above left = #2 and 3*(#3/5), nospace](#1_left_group_right_node){};
\node at (#1.center) [above right = #2 and 3*(#3/5), nospace](#1_right_group_left_node){};
\node at (#1.center) [above left = #2 and #3/5, nospace](#1_center_group_left_node){};
\node at (#1.center) [above right = #2 and #3/5, nospace](#1_center_group_right_node){};
}

\newcommand{\whyntreeboxbordersabstract}[3]{
% 1 = principal node
% 2 = tree height
% 3 = tree base length/2

% boxline up right
\node at (#1_left_group_right_node.center) [below right = #2/4 and #3/10, nospace](#1_leftupboxrightnode){};
\node at (#1_leftupboxrightnode.center) [left= 2*#3/5, nospace](#1_leftupboxleftnode){};
\draw[exboxline](#1_leftupboxrightnode)to(#1_leftupboxleftnode);

% boxline left
\node at (#1_right_group_left_node.center) [below left = #2/2 and 3*#3/10, nospace](#1_rightupboxrightnode){};
\node at (#1_rightupboxrightnode.center) [right= 2*#3/5, nospace](#1_rightupboxleftnode){};
\draw[exboxline](#1_rightupboxrightnode)to(#1_rightupboxleftnode);

% boxline below right
\node at (#1.center) [above left= #2/4 and #3/20, nospace](#1_leftdownboxrightnode){};
\node at (#1_leftdownboxrightnode.center) [left= 2*#3/5, nospace](#1_leftdownboxleftnode){};
\draw[exboxline](#1_leftdownboxrightnode)to(#1_leftdownboxleftnode);

}

\newcommand{\whyntreeweakeningleavesontheleft}[1]{
% 1 = principal node
\node at (#1_left_vertex.center) [above=\hstalt, etic](#1_weak1){\tiny $\weak$};
\node at (#1_left_group_right_node.center) [above=\hstalt, etic](#1_weakn){\tiny $\weak$};

\draw[nopol](#1_weak1) to (#1_left_vertex);
\draw[nopol](#1_weakn) to (#1_left_group_right_node);

\gdots{#1_left_vertex}{#1_left_group_right_node}{above = 2pt}
}

\newcommand{\whyntreeleavesabstract}[3]{
% 1 = principal node
% 2 = tree height
% 3 = tree base length/2

% derelictions
\node at (#1_center_group_left_node.center) [above=\hstalt, etic](#1_dern){\tiny $\der$};
\node at (#1_center_group_right_node.center) [above=\hstalt, etic](#1_der1){\tiny $\der$};

\draw[nopol](#1_dern) to (#1_center_group_left_node);
\draw[nopol](#1_der1) to (#1_center_group_right_node);

\gdots{#1_center_group_left_node}{#1_center_group_right_node}{above = 2pt}

%weakening
\whyntreeweakeningleavesontheleft{#1}

% axioms
\node at (#1_right_vertex.center) [above right=\hstalt and #3/4, etic](#1_ax1){\tiny $\ax$};
\node at (#1_right_vertex.center) [right=2*#3/4, nospace](#1_ax1_ghost_concl){};
\draw[nopol, out = 180, in = 90](#1_ax1) to (#1_right_vertex);
\draw[nopol, out = 0, in = 90](#1_ax1) to (#1_ax1_ghost_concl);

\node at (#1_ax1.center) [above=3*\hstalt/4, etic](#1_axn){\tiny $\ax$};
\node at (#1_right_group_left_node.center) [right=13*#3/10, nospace](#1_axn_ghost_concl){};

\draw[nopol, out = 180, in = 90, looseness=1.8](#1_axn) to (#1_right_group_left_node);
\draw[nopol, out = 0, in = 90, looseness=1.8](#1_axn) to (#1_axn_ghost_concl);

\gdots{#1_right_vertex}{#1_right_group_left_node}{above = 2pt}

}

\newcommand{\whyntree}[1]{
% 1 = principal node
\whyntreeabstract{#1}{\whyntreeheigth}{\whyntreelength}
}

\newcommand{\whyntreeboxborders}[1]{
% 1 = principal node
\whyntreeabstract{#1}{\whyntreeheigth}{\whyntreelength}
\whyntreeboxbordersabstract{#1}{\whyntreeheigth}{\whyntreelength}
}

\newcommand{\whyntreeboxbordersleaves}[1]{
% 1 = principal node
\whyntreeboxborders{#1}{\whyntreeheigth}{\whyntreelength}
\whyntreeleavesabstract{#1}{\whyntreeheigth}{\whyntreelength}
}

\newcommand{\whyntreeboxbordersleaveswithpremises}[1]{
% 1 = principal node

\whyntreeboxbordersleaves{#1}

% dereliction premises
\node at (#1_der1.center) [above=\hstalt, nospace](#1_der1_premise){};
\node at (#1_dern.center) [above=\hstalt, nospace](#1_dern_premise){};
\draw[nopol](#1_der1_premise) to (#1_der1);
\draw[nopol](#1_dern_premise) to (#1_dern);
}

%%%%%%%%%%%%%%%%
%% BOX BORDERS
%%%%%%%%%%%%%%%
\newcommand{\boxdershorizontaldistance}{7pt}
\newcommand{\boxdersverticaldistance}{2pt}
\newcommand{\boxdersdots}{5pt}

\newcommand{\boxcornerright}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

% internal box
\node at (#1.center)[left=#2, nospace](#1lineaso){};
\node at (#1.center)[above=#3, nospace](#1lineane){};
\draw[#4](#1lineaso.center) -- (#1.center) -- (#1lineane.center);

% internal box dotted extensions
\node at (#1lineaso.center)[left=\boxdersdots, nospace](#1lineasodotted){};
\node at (#1lineane.center)[above=\boxdersdots, nospace](#1lineanedotted){};
\draw[#4, densely dotted](#1lineaso)to(#1lineasodotted);
\draw[#4, densely dotted](#1lineane)to(#1lineanedotted);
}


\newcommand{\boxcornersright}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline
\node at (#1.center)[above right=2pt and 4pt, etic](#1dots){\tiny $...$};
\boxcornerright{#1}{#2}{#3}{#4}

% external box
\node at (#1.center)[below right=\boxdersverticaldistance and \boxdershorizontaldistance, nospace](#1linease2){};
\node at (#1lineaso.center)[below=\boxdersverticaldistance, nospace](#1lineaso2){};

\node at (#1lineane.center)[right=\boxdershorizontaldistance, nospace](#1lineane2){};
\draw[#4](#1lineaso2.center) -- (#1linease2.center) -- (#1lineane2.center);

% external box dotted extensions
\node at (#1lineaso2.center)[left=\boxdersdots, nospace](#1lineaso2dotted){};
\node at (#1lineane2.center)[above=\boxdersdots, nospace](#1lineane2dotted){};
\draw[#4, densely dotted](#1lineaso2)to(#1lineaso2dotted);
\draw[#4, densely dotted](#1lineane2)to(#1lineane2dotted);



}

\newcommand{\boxcornerleft}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

% internal box
\node at (#1.center)[right=#2, nospace](#1lineaso){};
\node at (#1.center)[above=#3, nospace](#1lineane){};
\draw[#4](#1lineaso.center) -- (#1.center) -- (#1lineane.center);

% internal box dotted extensions
\node at (#1lineaso.center)[right=\boxdersdots, nospace](#1lineasodotted){};
\node at (#1lineane.center)[above=\boxdersdots, nospace](#1lineanedotted){};
\draw[#4, densely dotted](#1lineaso)to(#1lineasodotted);
\draw[#4, densely dotted](#1lineane)to(#1lineanedotted);
}

\newcommand{\boxcornersleft}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

\node at (#1.center)[above left=2pt and 4pt, etic](#1dots){\tiny $...$};

\boxcornerleft{#1}{#2}{#3}{#4}

% external box
\node at (#1.center)[below left=\boxdersverticaldistance and \boxdershorizontaldistance, nospace](#1linease2){};
\node at (#1lineaso.center)[below=\boxdersverticaldistance, nospace](#1lineaso2){};

\node at (#1lineane.center)[left=\boxdershorizontaldistance, nospace](#1lineane2){};
\draw[#4](#1lineaso2.center) -- (#1linease2.center) -- (#1lineane2.center);

% external box dotted extensions
\node at (#1lineaso2.center)[right=\boxdersdots, nospace](#1lineaso2dotted){};
\node at (#1lineane2.center)[above=\boxdersdots, nospace](#1lineane2dotted){};
\draw[#4, densely dotted](#1lineaso2)to(#1lineaso2dotted);
\draw[#4, densely dotted](#1lineane2)to(#1lineane2dotted);



}


==> latex-macros/graphical-macros/links-MELL.tex <==
\newcommand{\lax}[3]{
% 1 = left port
% 2 = right port
% 3 = link name
\laxabstract{#1}{#2}{#3}{\altax}{\tiny}{nopol}{nopol}}

\newcommand{\lcut}[3]{
% 1 = left port
% 2 = right port
% 3 = link name
\lcutabstract{#1}{#2}{#3}{\altcut}{\tiny}{nopol}{nopol}}


%%%%%%%%
%% MULTIPLICATIVES
%%%%%%%%

\newcommand{\ltens}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinary{#1}{#2}{#3}{#4}{$\tens$}{nopol}}

\newcommand{\lpar}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinary{#1}{#2}{#3}{#4}{$\parr$}{nopol}}

\newcommand{\lone}[2]{
% 1 = one principal port	
% 2 = name of the link
\lzeroary{#1}{#2}{$\one$}{\hstalt}{nopol}}

\newcommand{\lbot}[2]{
% 1 = one principal port	
% 2 = name of the link
\lzeroary{#1}{#2}{$\bot$}{\hstalt}{nopol}}


%%%%%%%%
%% EXPONENTIALS
%%%%%%%%

\newcommand{\lder}[3]{
% parameters
% 1 = principal port	
% 2 = auxiliary port	
% 3 = name of the link
\lUnary{#1}{#2}{#3}{$\der$}{nopol}
}

\newcommand{\lbang}[3]{
% parameters
% 1 = principal port	
% 2 = auxiliary port	
% 3 = name of the link
\lUnary{#1}{#2}{#3}{$\bang$}{nopol}
}

\newcommand{\lweak}[2]{
% 1 = one principal port	
% 2 = name of the link
\lZeroary{#1}{#2}{$\weak$}{1.3*\hstalt}{nopol}
}

\newcommand{\lcontr}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinary{#1}{#2}{#3}{#4}{$\contr$}{nopol}}



